Inflation, (P)reheating and Neutrino Anomalies: Production of Sterile Neutrinos with Secret Interactions

A number of experimental anomalies involving neutrinos hint towards the existence of at least an extra (a very light) sterile neutrino. However, such a species, appreciably mixing with the active neutrinos, is disfavored by different cosmological observations like Big Bang Nucleosynthesis (BBN), Cosmic Microwave Background (CMB) and Large Scale Structure (LSS). Recently, it was shown that the presence of additional interactions in the sterile neutrino sector via light bosonic mediators can make the scenario cosmologically viable by suppressing the production of the sterile neutrinos from active neutrinos via matter-like effect caused by the mediator. This mechanism works assuming the initial population of this sterile sector to be negligible with respect to that of the Standard Model (SM) particles, before the production from active neutrinos. However, there is fair chance that such bosonic mediators may couple to the inflaton and can be copiously produced during (p)reheating epoch. Consequently, they may ruin this assumption of initial small density of the sterile sector. In this article we, starting from inflation, investigate the production of such a sterile sector during (p)reheating in a large field inflationary scenario and identify the parameter region that allows for a viable early Universe cosmology.

==> Bibliography.tex <==
\medskip


\begin{thebibliography}{00}
%-------------------------------------------


%LSND---------------------------------------- 
%\cite{Athanassopoulos:1995iw}
\bibitem{Athanassopoulos:1995iw}
C.~Athanassopoulos {\it et al.} [LSND Collaboration],
%``Candidate events in a search for anti-muon-neutrino ---> anti-electron-neutrino oscillations,''
Phys.\ Rev.\ Lett.\  {\bf 75} (1995) 2650
%doi:10.1103/PhysRevLett.75.2650
[nucl-ex/9504002].
%%CITATION = doi:10.1103/PhysRevLett.75.2650;%%
%723 citations counted in INSPIRE as of 06 Aug 2018

%\cite{Aguilar:2001ty}
\bibitem{Aguilar:2001ty}
A.~Aguilar-Arevalo {\it et al.} [LSND Collaboration],
%``Evidence for neutrino oscillations from the observation of anti-neutrino(electron) appearance in a anti-neutrino(muon) beam,''
Phys.\ Rev.\ D {\bf 64} (2001) 112007
%doi:10.1103/PhysRevD.64.112007
[hep-ex/0104049].
%%CITATION = doi:10.1103/PhysRevD.64.112007;%%
%1748 citations counted in INSPIRE as of 06 Aug 2018

%MiniBoone-------------------------------------------
%\cite{Aguilar-Arevalo:2018gpe}
%\bibitem{Aguilar-Arevalo:2018gpe}
%A.~A.~Aguilar-Arevalo {\it et al.} [MiniBooNE Collaboration],
%``Observation of a Significant Excess of Electron-Like Events in the MiniBooNE Short-Baseline Neutrino Experiment,''
%arXiv:1805.12028 [hep-ex].
%%CITATION = ARXIV:1805.12028;%%
%11 citations counted in INSPIRE as of 06 Aug 2018

%\cite{Aguilar-Arevalo:2018gpe}
\bibitem{Aguilar-Arevalo:2018gpe}
A.~A.~Aguilar-Arevalo {\it et al.} [MiniBooNE Collaboration],
%``Significant Excess of ElectronLike Events in the MiniBooNE Short-Baseline Neutrino Experiment,''
Phys.\ Rev.\ Lett.\  {\bf 121} (2018) no.22,  221801
%doi:10.1103/PhysRevLett.121.221801
[arXiv:1805.12028 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevLett.121.221801;%%
%53 citations counted in INSPIRE as of 14 Dec 2018


%mini-Sci mu_nu disapp-------------------------------------
%\cite{Cheng:2012yy}
%\bibitem{Cheng:2012yy}
%G.~Cheng {\it et al.} [MiniBooNE and SciBooNE Collaborations],
%``Dual baseline search for muon antineutrino disappearance at $0.1 {\rm eV}^2 < {\Delta}m^2 < 100 {\rm eV}^2$,''
%Phys.\ Rev.\ D {\bf 86} (2012) 052009
%doi:10.1103/PhysRevD.86.052009
%[arXiv:1208.0322 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevD.86.052009;%%
%106 citations counted in INSPIRE as of 19 Aug 2018

%\cite{Mahn:2011ea}
%\bibitem{Mahn:2011ea}
%K.~B.~M.~Mahn {\it et al.} [SciBooNE and MiniBooNE %Collaborations],
%``Dual baseline search for muon neutrino disappearance at $0.5 {\rm eV}^2 < \Delta m^2 < 40 {\rm eV}^2$,''
%Phys.\ Rev.\ D {\bf 85} (2012) 032007
%doi:10.1103/PhysRevD.85.032007
%[arXiv:1106.5685 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevD.85.032007;%%
%105 citations counted in INSPIRE as of 19 Aug 2018

%\cite{An:2016luf}
\bibitem{An:2016luf}
F.~P.~An {\it et al.} [Daya Bay Collaboration],
%``Improved Search for a Light Sterile Neutrino with the Full Configuration of the Daya Bay Experiment,''
Phys.\ Rev.\ Lett.\  {\bf 117} (2016) no.15,  151802
%doi:10.1103/PhysRevLett.117.151802
[arXiv:1607.01174 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevLett.117.151802;%%
%44 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Ko:2016owz}
\bibitem{Ko:2016owz}
Y.~J.~Ko {\it et al.} [NEOS Collaboration],
%``Sterile Neutrino Search at the NEOS Experiment,''
Phys.\ Rev.\ Lett.\  {\bf 118} (2017) no.12,  121802
%doi:10.1103/PhysRevLett.118.121802
[arXiv:1610.05134 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevLett.118.121802;%%
%68 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Alekseev:2016llm}
\bibitem{Alekseev:2016llm}
I.~Alekseev {\it et al.},
%``DANSS: Detector of the reactor AntiNeutrino based on Solid Scintillator,''
JINST {\bf 11} (2016) no.11,  P11011
%doi:10.1088/1748-0221/11/11/P11011
[arXiv:1606.02896 [physics.ins-det]].
%%CITATION = doi:10.1088/1748-0221/11/11/P11011;%%
%44 citations counted in INSPIRE as of 20 Aug 2018

%Reactor------------------------------------------------------
%\cite{Mention:2011rk}
\bibitem{Mention:2011rk}
G.~Mention, M.~Fechner, T.~Lasserre, T.~A.~Mueller, D.~Lhuillier, M.~Cribier and A.~Letourneau,
%``The Reactor Antineutrino Anomaly,''
Phys.\ Rev.\ D {\bf 83} (2011) 073006
%doi:10.1103/PhysRevD.83.073006
[arXiv:1101.2755 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevD.83.073006;%%
%966 citations counted in INSPIRE as of 06 Aug 2018

%\cite{Mueller:2011nm}
\bibitem{Mueller:2011nm}
T.~A.~Mueller {\it et al.},
%``Improved Predictions of Reactor Antineutrino Spectra,''
Phys.\ Rev.\ C {\bf 83} (2011) 054615
%doi:10.1103/PhysRevC.83.054615
[arXiv:1101.2663 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevC.83.054615;%%
%696 citations counted in INSPIRE as of 06 Aug 2018

%\cite{Huber:2011wv}
\bibitem{Huber:2011wv}
P.~Huber,
%``On the determination of anti-neutrino spectra from nuclear reactors,''
Phys.\ Rev.\ C {\bf 84} (2011) 024617
Erratum: [Phys.\ Rev.\ C {\bf 85} (2012) 029901]
%doi:10.1103/PhysRevC.85.029901,10.1103/PhysRevC.84.024617
[arXiv:1106.0687 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevC.85.029901, 10.1103/PhysRevC.84.024617;%%
%543 citations counted in INSPIRE as of 06 Aug 2018

%Gallium--------------------------------------------
%\cite{Laveder:2007zz}
\bibitem{Laveder:2007zz}
M.~Laveder,
%``Unbound neutrino roadmaps,''
Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 168} (2007) 344.
%doi:10.1016/j.nuclphysbps.2007.02.037
%%CITATION = doi:10.1016/j.nuclphysbps.2007.02.037;%%
%60 citations counted in INSPIRE as of 06 Aug 2018

%\cite{Giunti:2006bj}
\bibitem{Giunti:2006bj}
C.~Giunti and M.~Laveder,
%``Short-Baseline Active-Sterile Neutrino Oscillations?,''
Mod.\ Phys.\ Lett.\ A {\bf 22} (2007) 2499
%doi:10.1142/S0217732307025455
[hep-ph/0610352].
%%CITATION = doi:10.1142/S0217732307025455;%%
%99 citations counted in INSPIRE as of 06 Aug 2018


%\cite{Giunti:2010zu}
\bibitem{Giunti:2010zu}
C.~Giunti and M.~Laveder,
%``Statistical Significance of the Gallium Anomaly,''
Phys.\ Rev.\ C {\bf 83} (2011) 065504
%doi:10.1103/PhysRevC.83.065504
[arXiv:1006.3244 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevC.83.065504;%%
%332 citations counted in INSPIRE as of 06 Aug 2018

%GALLEX----------------------------------------------
%\cite{Kaether:2010ag}
\bibitem{Kaether:2010ag}
F.~Kaether, W.~Hampel, G.~Heusser, J.~Kiko and T.~Kirsten,
%``Reanalysis of the GALLEX solar neutrino flux and source experiments,''
Phys.\ Lett.\ B {\bf 685} (2010) 47
%doi:10.1016/j.physletb.2010.01.030
[arXiv:1001.2731 [hep-ex]].
%%CITATION = doi:10.1016/j.physletb.2010.01.030;%%
%293 citations counted in INSPIRE as of 06 Aug 2018

%SAGE--------------------------------------------------
%\cite{Abdurashitov:2009tn}
\bibitem{Abdurashitov:2009tn}
J.~N.~Abdurashitov {\it et al.} [SAGE Collaboration],
%``Measurement of the solar neutrino capture rate with gallium metal. III: Results for the 2002--2007 data-taking period,''
Phys.\ Rev.\ C {\bf 80} (2009) 015807
%doi:10.1103/PhysRevC.80.015807
[arXiv:0901.2200 [nucl-ex]].
%%CITATION = doi:10.1103/PhysRevC.80.015807;%%
%452 citations counted in INSPIRE as of 06 Aug 2018

%MINOS and +-------------------------------------------------
%\cite{Adamson:2017uda}
\bibitem{Adamson:2017uda}
P.~Adamson {\it et al.} [MINOS Collaboration],
%``Search for sterile neutrinos in MINOS and MINOS+ using a two-detector fit,''
%Submitted to: Phys.Rev.Lett.
[arXiv:1710.06488 [hep-ex]].
%%CITATION = ARXIV:1710.06488;%%
%8 citations counted in INSPIRE as of 19 Aug 2018

%ICECUBE--------------------------------------------
%\cite{TheIceCube:2016oqi}
\bibitem{TheIceCube:2016oqi}
M.~G.~Aartsen {\it et al.} [IceCube Collaboration],
%``Searches for Sterile Neutrinos with the IceCube Detector,''
Phys.\ Rev.\ Lett.\  {\bf 117} (2016) no.7,  071801
%doi:10.1103/PhysRevLett.117.071801
[arXiv:1605.01990 [hep-ex]].
%%CITATION = doi:10.1103/PhysRevLett.117.071801;%%
%115 citations counted in INSPIRE as of 19 Aug 2018



%--------------------------------------------------
%----------------------------------------------------
%---------------------------------------------------
%-----------------------------------------------------

%\cite{Dentler:2018sju}
\bibitem{Dentler:2018sju}
M.~Dentler \textit{et al.}, %, Á.~Hernandez~Cabezudo, J.~Kopp, P.~Machado, M.~Maltoni, I.~Martinez~Soler and T.~Schwetz,
%``Updated Global Analysis of Neutrino Oscillations in the Presence of eV-Scale Sterile Neutrinos,''
JHEP {\bf 1808} (2018) 010
%doi:10.1007/JHEP08(2018)010
[arXiv:1803.10661 [hep-ph]].
%%CITATION = doi:10.1007/JHEP08(2018)010;%%
%22 citations counted in INSPIRE as of 18 Aug 2018


%\cite{Doring:2018cob}
\bibitem{Doring:2018cob} 
  D.~Doring, H.~Pas, P.~Sicking and T.~J.~Weiler,
  %``Sterile Neutrinos with Altered Dispersion Relations as an Explanation for the MiniBooNE, LSND, Gallium and Reactor Anomalies,''
  arXiv:1808.07460 [hep-ph].
  %%CITATION = ARXIV:1808.07460;%%

  %\cite{Barbieri:1990vx}
\bibitem{Barbieri:1990vx} 
R.~Barbieri and A.~Dolgov,
%``Neutrino oscillations in the early universe,''
Nucl.\ Phys.\ B {\bf 349}, 743 (1991).
%doi:10.1016/0550-3213(91)90396-F
%%CITATION = doi:10.1016/0550-3213(91)90396-F;%%
%242 citations counted in INSPIRE as of 25 Aug 2018

%\cite{Enqvist:1990ad}
\bibitem{Enqvist:1990ad} 
K.~Enqvist, K.~Kainulainen and J.~Maalampi,
%``Refraction and Oscillations of Neutrinos in the Early Universe,''
Nucl.\ Phys.\ B {\bf 349}, 754 (1991).
% doi:10.1016/0550-3213(91)90397-G
%%CITATION = doi:10.1016/0550-3213(91)90397-G;%%
%175 citations counted in INSPIRE as of 25 Aug 2018

%@article{BARBIERI1990440,
%	title = "Bounds on sterile neutrinos from nucleosynthesis",
%	journal = "Physics Letters B",
%	volume = "237",
%	number = "3",
%	pages = "440 - 445",
%	year = "1990",
%	issn = "0370-2693",
%	doi = "https://doi.org/10.1016/0370-2693(90)91203-N",
%	url = "http://www.sciencedirect.com/science/article/pii/037026939091203N",
%	author = "R. Barbieri and A. Dolgov",
	
%}

%\cite{BARBIERI1990440}
\bibitem{BARBIERI1990440}
R. Barbieri and A. Dolgov,
%``Bounds on sterile neutrinos from nucleosynthesis,''
Physics Letters B {\bf 237} (1990) 440.


%\cite{Enqvist:1991qj}
%\bibitem{Enqvist:1991qj}
%K.~Enqvist, K.~Kainulainen and M.~J.~Thomson,
%``Stringent cosmological bounds on inert neutrino mixing,''
%Nucl.\ Phys.\ B {\bf 373} (1992) 498.
%doi:10.1016/0550-3213(92)90442-E
%%CITATION = doi:10.1016/0550-3213(92)90442-E;%%
%279 citations counted in INSPIRE as of 29 Jan 2019

%\cite{Kainulainen:1990ds}
\bibitem{Kainulainen:1990ds}
K.~Kainulainen,
%``Light Singlet Neutrinos and the Primordial Nucleosynthesis,''
Phys.\ Lett.\ B {\bf 244} (1990) 191.
%doi:10.1016/0370-2693(90)90054-A
%%CITATION = doi:10.1016/0370-2693(90)90054-A;%%
%167 citations counted in INSPIRE as of 29 Jan 2019



%\cite{Dodelson:1993je}
\bibitem{Dodelson:1993je}
S.~Dodelson and L.~M.~Widrow,
%``Sterile-neutrinos as dark matter,''
Phys.\ Rev.\ Lett.\  {\bf 72} (1994) 17
%doi:10.1103/PhysRevLett.72.17
[hep-ph/9303287].
%%CITATION = doi:10.1103/PhysRevLett.72.17;%%
%809 citations counted in INSPIRE as of 19 Aug 2018

%\cite{Merle:2015vzu}
\bibitem{Merle:2015vzu}
A.~Merle, A.~Schneider and M.~Totzauer,
%``Dodelson-Widrow Production of Sterile Neutrino Dark Matter with Non-Trivial Initial Abundance,''
JCAP {\bf 1604} (2016) no.04,  003
%doi:10.1088/1475-7516/2016/04/003
[arXiv:1512.05369 [hep-ph]].
%%CITATION = doi:10.1088/1475-7516/2016/04/003;%%
%27 citations counted in INSPIRE as of 21 Aug 2018


%\cite{Shaposhnikov:2006xi}
\bibitem{Shaposhnikov:2006xi}
M.~Shaposhnikov and I.~Tkachev,
%``The nuMSM, inflation, and dark matter,''
Phys.\ Lett.\ B {\bf 639} (2006) 414
%doi:10.1016/j.physletb.2006.06.063
[hep-ph/0604236].
%%CITATION = doi:10.1016/j.physletb.2006.06.063;%%
%287 citations counted in INSPIRE as of 19 Aug 2018

%\cite{Merle:2013wta}
\bibitem{Merle:2013wta}
A.~Merle, V.~Niro and D.~Schmidt,
%``New Production Mechanism for keV Sterile Neutrino Dark Matter by Decays of Frozen-In Scalars,''
JCAP {\bf 1403} (2014) 028
%doi:10.1088/1475-7516/2014/03/028
[arXiv:1306.3996 [hep-ph]].
%%CITATION = doi:10.1088/1475-7516/2014/03/028;%%
%87 citations counted in INSPIRE as of 21 Aug 2018

%\cite{Kusenko:2006rh}
\bibitem{Kusenko:2006rh}
A.~Kusenko,
%``Sterile neutrinos, dark matter, and the pulsar velocities in models with a Higgs singlet,''
Phys.\ Rev.\ Lett.\  {\bf 97} (2006) 241301
%doi:10.1103/PhysRevLett.97.241301
[hep-ph/0609081].
%%CITATION = doi:10.1103/PhysRevLett.97.241301;%%
%225 citations counted in INSPIRE as of 21 Aug 2018


%\cite{Cooke:2013cba}
\bibitem{Cooke:2013cba}
R.~Cooke, M.~Pettini, R.~A.~Jorgenson, M.~T.~Murphy and C.~C.~Steidel,
%``Precision measures of the primordial abundance of deuterium,''
Astrophys.\ J.\  {\bf 781} (2014) no.1,  31
%doi:10.1088/0004-637X/781/1/31
[arXiv:1308.3240 [astro-ph.CO]].
%%CITATION = doi:10.1088/0004-637X/781/1/31;%%
%227 citations counted in INSPIRE as of 17 Aug 2018

%\cite{pdg18}
\bibitem{pdg18}
 M.~Tanabashi \textit{et al.} (Particle Data Group),
 %Phys. Rev. D 98, 030001 (2018).
Phys.\ Rev.\ D {\bf 98} (2018) 030001

%\cite{Cooke:2017cwo}
\bibitem{Cooke:2017cwo}
R.~J.~Cooke, M.~Pettini and C.~C.~Steidel,
%``One Percent Determination of the Primordial Deuterium Abundance,''
Astrophys.\ J.\  {\bf 855} (2018) no.2,  102
%doi:10.3847/1538-4357/aaab53
[arXiv:1710.11129 [astro-ph.CO]].
%%CITATION = doi:10.3847/1538-4357/aaab53;%%
%17 citations counted in INSPIRE as of 21 Aug 2018

\bibitem{BBN}
G.~Mangano and P.~D.~Serpico,
%``A robust upper limit on N$_{}$ from BBN, circa 2011,''
Physics Letters  B {\bf 701} (July, 2011) 296--299.
%doi:10.1016/j.physletb.2011.05.075
[arXiv:1103.1261 [astro-ph.CO]].

%------------------------------------------------------
%\cite{nucos}
\bibitem{nucos}
J.~Lesgourgues, G.~Mangano, G.~Miele, S.~Pastor,
``Neutrino Cosmology'',
Cambridge University Press

%\cite{silk}
\bibitem{silk}
J.R.~Bond  {\it et al.},
 Phys.\ Rev.\ Lett.\  {\bf 45}(1980)


%\cite{Alam:2016hwk}
\bibitem{Alam:2016hwk}
S.~Alam {\it et al.} [BOSS Collaboration],
%``The clustering of galaxies in the completed SDSS-III Baryon Oscillation Spectroscopic Survey: cosmological analysis of the DR12 galaxy sample,''
Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 470} (2017) no.3,  2617
%doi:10.1093/mnras/stx721
[arXiv:1607.03155 [astro-ph.CO]].
%%CITATION = doi:10.1093/mnras/stx721;%%
%331 citations counted in INSPIRE as of 21 Aug 2018


%\cite{Zarrouk:2018vwy}
\bibitem{Zarrouk:2018vwy}
P.~Zarrouk {\it et al.},
%``The clustering of the SDSS-IV extended Baryon Oscillation Spectroscopic Survey DR14 quasar sample: measurement of the growth rate of structure from the anisotropic correlation function between redshift 0.8 and 2.2,''
Mon.\ Not.\ Roy.\ Astron.\ Soc.\  {\bf 477} (2018) no.2,  1639
%doi:10.1093/mnras/sty506
[arXiv:1801.03062 [astro-ph.CO]].
%%CITATION = doi:10.1093/mnras/sty506;%%
%7 citations counted in INSPIRE as of 20 Aug 2018

%\cite{boss}
\bibitem{boss}
K.S.~Dawson {\it et al.},
%The  Baryon  Oscillation Spectroscopic Survey of SDSS-III. 2013, 
\ AJ, {\bf 145}, 10, 2013
[arXiv:1208.0022 [astro-ph.CO]]

%\cite{Palanque-Delabrouille:2015pga}
\bibitem{Palanque-Delabrouille:2015pga}
N.~Palanque-Delabrouille {\it et al.},
%``Neutrino masses and cosmology with Lyman-alpha forest power spectrum,''
JCAP {\bf 1511} (2015) no.11,  011
%doi:10.1088/1475-7516/2015/11/011
[arXiv:1506.05976 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2015/11/011;%%
%137 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Yeche:2017upn}
\bibitem{Yeche:2017upn}
C.~Yeche, N.~Palanque-Delabrouille, J.~Baur and H.~du Mas des Bourboux,
%``Constraints on neutrino masses from Lyman-alpha forest power spectrum with BOSS and XQ-100,''
JCAP {\bf 1706} (2017) no.06,  047
%doi:10.1088/1475-7516/2017/06/047
[arXiv:1702.03314 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2017/06/047;%%
%38 citations counted in INSPIRE as of 20 Aug 2018


%\cite{Mangano:2001iu}
\bibitem{Mangano:2001iu}
G.~Mangano, G.~Miele, S.~Pastor and M.~Peloso,
%``A Precision calculation of the effective number of cosmological neutrinos,''
Phys.\ Lett.\ B {\bf 534} (2002) 8
%doi:10.1016/S0370-2693(02)01622-2
[astro-ph/0111408].
%%CITATION = doi:10.1016/S0370-2693(02)01622-2;%%
%164 citations counted in INSPIRE as of 21 Aug 2018

%\bibitem{Kopp:2013vaa} 
%  J.~Kopp, P.~A.~N.~Machado, M.~Maltoni and T.~Schwetz,
  %``Sterile Neutrino Oscillations: The Global Picture,''
 % JHEP {\bf 1305}, 050 (2013)
  %[arXiv:1303.3011 [hep-ph]].
  %%CITATION = ARXIV:1303.3011;%%
  %38 citations counted in INSPIRE as of 11 Oct 2013
  
  
%\cite{Giunti:2012tn}
%\bibitem{Giunti:2012tn}
%C.~Giunti, M.~Laveder, Y.~F.~Li, Q.~Y.~Liu and H.~W.~Long,
%``Update of Short-Baseline Electron Neutrino and Antineutrino Disappearance,''
%Phys.\ Rev.\ D {\bf 86} (2012) 113014
%doi:10.1103/PhysRevD.86.113014
%[arXiv:1210.5715 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevD.86.113014;%%
%158 citations counted in INSPIRE as of 06 Aug 2018

%\cite{Vagnozzi:2017ovm}
\bibitem{Vagnozzi:2017ovm}
S.~Vagnozzi, E.~Giusarma, O.~Mena, K.~Freese, M.~Gerbino, S.~Ho and M.~Lattanzi,
%``Unveiling $\nu$ secrets with cosmological data: neutrino masses and mass hierarchy,''
Phys.\ Rev.\ D {\bf 96} (2017) no.12,  123503
%doi:10.1103/PhysRevD.96.123503
arXiv:1701.08172 [astro-ph.CO].
%%CITATION = doi:10.1103/PhysRevD.96.123503;%%
%82 citations counted in INSPIRE as of 23 Jan 2019


%\cite{Aghanim:2018eyx}
\bibitem{Aghanim:2018eyx}
N.~Aghanim {\it et al.} [Planck Collaboration],
%``Planck 2018 results. VI. Cosmological parameters,''
arXiv:1807.06209 [astro-ph.CO].
%%CITATION = ARXIV:1807.06209;%%
%31 citations counted in INSPIRE as of 16 Aug 2018


%\cite{Ade:2013zuv}
%\bibitem{Ade:2013zuv} 
 % P.~A.~R.~Ade {\it et al.},
  %``Planck 2013 results. XVI. Cosmological parameters,''
  %arXiv:1303.5076
  %%CITATION = ARXIV:1303.5076;%%
  %696 citations counted in INSPIRE as of 02 Oct 2013
 
 %\cite{Archidiacono:2013xxa}
 %\bibitem{Archidiacono:2013xxa}
% M.~Archidiacono, N.~Fornengo, C.~Giunti, S.~Hannestad and A.~Melchiorri,
 %``Sterile neutrinos: Cosmology versus short-baseline experiments,''
% Phys.\ Rev.\ D {\bf 87} (2013) no.12,  125034
% doi:10.1103/PhysRevD.87.125034
% [arXiv:1302.6720 [astro-ph.CO]].
 %%CITATION = doi:10.1103/PhysRevD.87.125034;%%
 %92 citations counted in INSPIRE as of 20 Aug 2018
  
  	
%\cite{Archidiacono:2013xxa}
%\bibitem{Archidiacono:2013xxa}
 % M.~Archidiacono, N.~Fornengo, C.~Giunti, S.~Hannestad and A.~Melchiorri,
  %``Sterile Neutrinos: Cosmology vs Short-BaseLine Experiments,''
%	Phys.\ Rev.\ D {\bf 87}, 125034 (2013).
  %arXiv:1302.6720 [astro-ph.CO].
  %%CITATION = ARXIV:1302.6720;%%
  %13 citations counted in INSPIRE as of 02 Oct 2013

%\cite{Canac:2016smv}
\bibitem{Canac:2016smv}
N.~Canac, G.~Aslanyan, K.~N.~Abazajian, R.~Easther and L.~C.~Price,
%``Testing for New Physics: Neutrinos and the Primordial Power Spectrum,''
JCAP {\bf 1609} (2016) no.09,  022
%doi:10.1088/1475-7516/2016/09/022
[arXiv:1606.03057 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2016/09/022;%%
%12 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Chudaykin:2014oia}
\bibitem{Chudaykin:2014oia}
A.~S.~Chudaykin, D.~S.~Gorbunov, A.~A.~Starobinsky and R.~A.~Burenin,
%``Cosmology based on f(R) gravity with Script O(1) eV sterile neutrino,''
JCAP {\bf 1505} (2015) no.05,  004
%doi:10.1088/1475-7516/2015/05/004
[arXiv:1412.5239 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2015/05/004;%%
%11 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Giusarma:2011zq}
\bibitem{Giusarma:2011zq}
E.~Giusarma, M.~Archidiacono, R.~de Putter, A.~Melchiorri and O.~Mena,
%``Sterile neutrino models and nonminimal cosmologies,''
Phys.\ Rev.\ D {\bf 85} (2012) 083522
%doi:10.1103/PhysRevD.85.083522
[arXiv:1112.4661 [astro-ph.CO]].
%%CITATION = doi:10.1103/PhysRevD.85.083522;%%
%39 citations counted in INSPIRE as of 28 Aug 2018

%\cite{Ho:2012br}
\bibitem{Ho:2012br}
C.~M.~Ho and R.~J.~Scherrer,
%``Sterile Neutrinos and Light Dark Matter Save Each Other,''
Phys.\ Rev.\ D {\bf 87} (2013) no.6,  065016
%doi:10.1103/PhysRevD.87.065016
[arXiv:1212.1689 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevD.87.065016;%%
%58 citations counted in INSPIRE as of 28 Aug 2018

%\cite{Chu:2006ua}
\bibitem{Chu:2006ua}
Y.~Z.~Chu and M.~Cirelli,
%``Sterile neutrinos, lepton asymmetries, primordial elements: How much of each?,''
Phys.\ Rev.\ D {\bf 74} (2006) 085015
%doi:10.1103/PhysRevD.74.085015
[astro-ph/0608206].
%%CITATION = doi:10.1103/PhysRevD.74.085015;%%
%58 citations counted in INSPIRE as of 28 Aug 2018

 \bibitem{Babu:1991at} 
K.~S.~Babu and I.~Z.~Rothstein,
%``Relaxing nucleosynthesis bounds on sterile-neutrinos,''
Phys.\ Lett.\ B {\bf 275}, 112 (1992).
%%CITATION = PHLTA,B275,112;%%
%24 citations counted in INSPIRE as of 03 Dec 2013

%\cite{Enqvist:1992}
\bibitem{Enqvist:1992} 
K.~Enqvist, K.~Kainulainen and M.~J.~Thomson,
%``Cosmological bounds on Dirac-Majorana neutrinos,''
Phys.\ Lett.\ B {\bf 280}, 245 (1992).
%%CITATION = PHLTA,B280,245;%%
%19 citations counted in INSPIRE as of 03 Dec 2013






  
  %\cite{Hannestad:2013ana}
\bibitem{Hannestad:2013ana} 
  S.~Hannestad, R.~S.~Hansen and T.~Tram,
  %``How Self-Interactions can Reconcile Sterile Neutrinos with Cosmology,''
  Phys.\ Rev.\ Lett.\  {\bf 112}, no. 3, 031802 (2014)
  %doi:10.1103/PhysRevLett.112.031802
  [arXiv:1310.5926 [astro-ph.CO]].
  %%CITATION = doi:10.1103/PhysRevLett.112.031802;%%
  %77 citations counted in INSPIRE as of 18 Mar 2018
 
  %\cite{Archidiacono:2014nda}
 \bibitem{Archidiacono:2014nda}
 M.~Archidiacono, S.~Hannestad, R.~S.~Hansen and T.~Tram,
 %``Cosmology with self-interacting sterile neutrinos and dark matter - A pseudoscalar model,''
 Phys.\ Rev.\ D {\bf 91} (2015) no.6,  065021
 %doi:10.1103/PhysRevD.91.065021
 [arXiv:1404.5915 [astro-ph.CO]].
 %%CITATION = doi:10.1103/PhysRevD.91.065021;%%
 %55 citations counted in INSPIRE as of 20 May 2018
 
 %\cite{Archidiacono:2015oma}
 \bibitem{Archidiacono:2015oma}
 M.~Archidiacono, S.~Hannestad, R.~S.~Hansen and T.~Tram,
 %``Sterile neutrinos with pseudoscalar self-interactions and cosmology,''
 Phys.\ Rev.\ D {\bf 93} (2016) no.4,  045004
 %doi:10.1103/PhysRevD.93.045004
 [arXiv:1508.02504 [astro-ph.CO]].
 %%CITATION = doi:10.1103/PhysRevD.93.045004;%%
 %16 citations counted in INSPIRE as of 03 Jul 2018

%\cite{Archidiacono:2016kkh}
\bibitem{Archidiacono:2016kkh}
M.~Archidiacono, S.~Gariazzo, C.~Giunti, S.~Hannestad, R.~Hansen, M.~Laveder and T.~Tram,
%``Pseudoscalar—sterile neutrino interactions: reconciling the cosmos with neutrino oscillations,''
JCAP {\bf 1608} (2016) no.08,  067
%doi:10.1088/1475-7516/2016/08/067
[arXiv:1606.07673 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2016/08/067;%%
%48 citations counted in INSPIRE as of 21 Aug 2018

%\cite{Kofman:1994rk}
\bibitem{Kofman:1994rk}
L.~Kofman, A.~D.~Linde and A.~A.~Starobinsky,
%``Reheating after inflation,''
Phys.\ Rev.\ Lett.\  {\bf 73} (1994) 3195
%doi:10.1103/PhysRevLett.73.3195
[hep-th/9405187].
%%CITATION = doi:10.1103/PhysRevLett.73.3195;%%
%1204 citations counted in INSPIRE as of 25 Jun 2018

%\cite{Kofman:1997yn}
\bibitem{Kofman:1997yn}
L.~Kofman, A.~D.~Linde and A.~A.~Starobinsky,
%``Towards the theory of reheating after inflation,''
Phys.\ Rev.\ D {\bf 56} (1997) 3258
%doi:10.1103/PhysRevD.56.3258
[hep-ph/9704452].
%%CITATION = doi:10.1103/PhysRevD.56.3258;%%
%1242 citations counted in INSPIRE as of 08 Sep 2018



 %\cite{Starobinsky:1994bd}
 \bibitem{Starobinsky:1994bd}
 A.~A.~Starobinsky and J.~Yokoyama,
 %``Equilibrium state of a selfinteracting scalar field in the De Sitter background,''
 Phys.\ Rev.\ D {\bf 50} (1994) 6357
 %doi:10.1103/PhysRevD.50.6357
 [astro-ph/9407016].
 %%CITATION = doi:10.1103/PhysRevD.50.6357;%%
 %378 citations counted in INSPIRE as of 21 Aug 2018
 
 
  %\cite{Akrami:2018odb}
 \bibitem{Akrami:2018odb}
 Y.~Akrami {\it et al.} [Planck Collaboration],
 %``Planck 2018 results. X. Constraints on inflation,''
 arXiv:1807.06211 [astro-ph.CO].
 %%CITATION = ARXIV:1807.06211;%%
 %13 citations counted in INSPIRE as of 16 Aug 2018

%\cite{linde:scalar}
\bibitem{linde:scalar}
A.D. Linde,
%Scalar field fluctuations in the expanding universe and the new inflationary universe scenario,
%Physics Letters B,
%Volume 116, Issue 5,
%1982,
%Pages 335-339,
Phys.\ Lett.\ B {\bf 116} (1982) 335
%ISSN 0370-2693,
%https://doi.org/10.1016/0370-2693(82)90293-3.
%(http://www.sciencedirect.com/science/article/pii/0370269382902933)

%\cite{star:scalar}
\bibitem{star:scalar} 
A.A. Starobinsky,
%Dynamics of phase transition in the new inflationary universe scenario and generation of perturbations,
Phys.\ Lett.\ B {\bf 117} (1982) 175
%Physics Letters B,
%Volume 117, Issues 3–4,
%1982,
%Pages 175-178,
%ISSN 0370-2693,
%https://doi.org/10.1016/0370-2693(82)90541-X.

 
%\cite{vile:scalar}
\bibitem{vile:scalar} 
A. Vilenkin and L.H. Ford,
Phys.\ Rev.\ D {\bf 26}, no. 6 (1982)

%\cite{Starobinsky:1994bd}
\bibitem{Starobinsky:1994bd}
A.~A.~Starobinsky and J.~Yokoyama,
%``Equilibrium state of a selfinteracting scalar field in the De Sitter background,''
Phys.\ Rev.\ D {\bf 50} (1994) 6357
%doi:10.1103/PhysRevD.50.6357
[astro-ph/9407016].
%%CITATION = doi:10.1103/PhysRevD.50.6357;%%
%401 citations counted in INSPIRE as of 06 Feb 2019


%@article{PhysRevD.26.1231,
%	title = {Gravitational effects upon cosmological phase transitions},
%	author = {Vilenkin, Alexander and Ford, L. H.},
%	journal = {Phys. Rev. D},
%	volume = {26},
%	issue = {6},
%	pages = {1231--1241},
%	numpages = {0},
%	year = {1982},
%	month = {Sep},
%	publisher = {American Physical Society},
%	doi = {10.1103/PhysRevD.26.1231},
%	url = {https://link.aps.org/doi/10.1103/PhysRevD.26.1231}
%}


  
  %\cite{Enqvist:2014zqa}
  \bibitem{Enqvist:2014zqa}
  K.~Enqvist, S.~Nurmi, T.~Tenkanen and K.~Tuominen,
  %``Standard Model with a real singlet scalar and inflation,''
  JCAP {\bf 1408} (2014) 035
 % doi:10.1088/1475-7516/2014/08/035
  [arXiv:1407.0659 [astro-ph.CO]].
  %%CITATION = doi:10.1088/1475-7516/2014/08/035;%%
  %29 citations counted in INSPIRE as of 20 Aug 2018
  
  
  %\cite{Dasgupta:2013zpn}
%\bibitem{Dasgupta:2013zpn} 
 % B.~Dasgupta and J.~Kopp,
  %``Cosmologically Safe eV-Scale Sterile Neutrinos and Improved Dark Matter Structure,''
 % Phys.\ Rev.\ Lett.\  {\bf 112}, no. 3, 031803 (2014)
  %doi:10.1103/PhysRevLett.112.031803
  %[arXiv:1310.6337 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.112.031803;%%
  %102 citations counted in INSPIRE as of 18 Mar 2018
  
 
%\cite{Patrignani:2016xqp}
%\bibitem{Patrignani:2016xqp} 
 % C.~Patrignani {\it et al.} [Particle Data Group],
  %``Review of Particle Physics,''
  %Chin.\ Phys.\ C {\bf 40}, no. 10, 100001 (2016).
  %doi:10.1088/1674-1137/40/10/100001
  %%CITATION = doi:10.1088/1674-1137/40/10/100001;%%
  %2843 citations counted in INSPIRE as of 19 Mar 2018
 
 
 %\cite{Lebedev:2012sy}
 %\bibitem{Lebedev:2012sy}
 %O.~Lebedev and A.~Westphal,
 %``Metastable Electroweak Vacuum: Implications for Inflation,''
 %Phys.\ Lett.\ B {\bf 719} (2013) 415
% doi:10.1016/j.physletb.2012.12.069
 %[arXiv:1210.6987 [hep-ph]].
 %%CITATION = doi:10.1016/j.physletb.2012.12.069;%%
 %77 citations counted in INSPIRE as of 21 Aug 2018
 
  
  %\cite{Dufaux:2006ee}
\bibitem{Dufaux:2006ee} 
  J.~F.~Dufaux, G.~N.~Felder, L.~Kofman, M.~Peloso and D.~Podolsky,
  %``Preheating with trilinear interactions: Tachyonic resonance,''
  JCAP {\bf 0607}, 006 (2006)
  %doi:10.1088/1475-7516/2006/07/006
  [hep-ph/0602144].
  %%CITATION = doi:10.1088/1475-7516/2006/07/006;%%
  %95 citations counted in INSPIRE as of 04 Apr 2018
  
  %\cite{Bezrukov:2008dt}
\bibitem{Bezrukov:2008dt} 
  F.~L.~Bezrukov,
  %``Non-minimal coupling in inflation and inflating with the Higgs boson,''
  arXiv:0810.3165 [hep-ph].
  %%CITATION = ARXIV:0810.3165;%%
  %12 citations counted in INSPIRE as of 04 Apr 2018

%\cite{Burgess:2009ea}
\bibitem{Burgess:2009ea}
C.~P.~Burgess, H.~M.~Lee and M.~Trott,
%``Power-counting and the Validity of the Classical Approximation During Inflation,''
JHEP {\bf 0909} (2009) 103
%doi:10.1088/1126-6708/2009/09/103
arXiv:0902.4465 [hep-ph].
%%CITATION = doi:10.1088/1126-6708/2009/09/103;%%
%251 citations counted in INSPIRE as of 24 Jan 2019

  
  %\cite{Bezrukov:2014ipa}
\bibitem{Bezrukov:2014ipa} 
  F.~Bezrukov, J.~Rubio and M.~Shaposhnikov,
  %``Living beyond the edge: Higgs inflation and vacuum metastability,''
  Phys.\ Rev.\ D {\bf 92}, no. 8, 083512 (2015)
  %doi:10.1103/PhysRevD.92.083512
  [arXiv:1412.3811 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.083512;%%
  %84 citations counted in INSPIRE as of 04 Apr 2018
  

  
   %\cite{Ade:2015lrj} 
 % \bibitem{Ade:2015lrj} P.~A.~R.~Ade {\it et al.} [Planck Collaboration], %``Planck 2015 results. XX. Constraints on inflation,''
  %Astron.\ Astrophys.\ {\bf 594}, A20 (2016)
  %doi:10.1051/0004-6361/201525898
  %[arXiv:1502.02114 [astro-ph.CO]].
  %%CITATION = doi:10.1051/0004-6361/201525898;%%
%1548 citations counted in INSPIRE as of 19 Mar 2018

%\cite{Kallosh:2013tua}
\bibitem{Kallosh:2013tua} 
  R.~Kallosh, A.~Linde and D.~Roest,
  %``Universal Attractor for Inflation at Strong Coupling,''
  Phys.\ Rev.\ Lett.\  {\bf 112}, no. 1, 011303 (2014)
  %doi:10.1103/PhysRevLett.112.011303
  [arXiv:1310.3950 [hep-th]].
  %%CITATION = doi:10.1103/PhysRevLett.112.011303;%%
  %168 citations counted in INSPIRE as of 19 Mar 2018
  
  %\cite{Linde:2011nh}
\bibitem{Linde:2011nh}
A.~Linde, M.~Noorbala and A.~Westphal,
%``Observational consequences of chaotic inflation with nonminimal coupling to gravity,''
JCAP {\bf 1103} (2011) 013
%doi:10.1088/1475-7516/2011/03/013
[arXiv:1101.2652 [hep-th]].
%%CITATION = doi:10.1088/1475-7516/2011/03/013;%%
%68 citations counted in INSPIRE as of 21 May 2018



  
  
  %\cite{Ghosh:2017fmr}
\bibitem{Ghosh:2017fmr} 
  P.~Ghosh, A.~K.~Saha and A.~Sil,
  %``Study of Electroweak Vacuum Stability from Extended Higgs Portal of Dark Matter and Neutrinos,''
  Phys.\ Rev.\ D {\bf 97}, no. 7, 075034 (2018)
  %doi:10.1103/PhysRevD.97.075034
  [arXiv:1706.04931 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.97.075034;%%
  %8 citations counted in INSPIRE as of 26 Aug 2018

%\cite{Ema:2017ckf}
\bibitem{Ema:2017ckf}
Y.~Ema, M.~Karciauskas, O.~Lebedev, S.~Rusak and M.~Zatta,
%``Higgs-Inflaton Mixing and Vacuum Stability,''
[arXiv:1711.10554 [hep-ph]].
%%CITATION = ARXIV:1711.10554;%%
%10 citations counted in INSPIRE as of 14 Dec 2018

%\cite{Khachatryan:2016whc}
%\bibitem{Khachatryan:2016whc}
%V.~Khachatryan {\it et al.} [CMS Collaboration],
%``Searches for invisible decays of the Higgs boson in pp collisions at $\sqrt{s}$ = 7, 8, and 13 TeV,''
%JHEP {\bf 1702} (2017) 135
%doi:10.1007/JHEP02(2017)135
%[arXiv:1610.09218 [hep-ex]].
%%CITATION = doi:10.1007/JHEP02(2017)135;%%
%107 citations counted in INSPIRE as of 28 Aug 2018

%\cite{sher}
\bibitem{sher}
Marc Sher,
%Electroweak Higgs potential and vacuum stability,
Physics Reports,
Volume \textbf{179}, Issues 5-6,
(1989),
Pages 273-418,
%ISSN 0370-1573,
%https://doi.org/10.1016/0370-1573(89)90061-6.
%(http://www.sciencedirect.com/science/article/pii/0370157389900616)

%\cite{EliasMiro:2011aa}
\bibitem{EliasMiro:2011aa}
J.~Elias-Miro, J.~R.~Espinosa, G.~F.~Giudice, G.~Isidori, A.~Riotto and A.~Strumia,
%``Higgs mass implications on the stability of the electroweak vacuum,''
Phys.\ Lett.\ B {\bf 709} (2012) 222
%doi:10.1016/j.physletb.2012.02.013
arXiv:1112.3022 [hep-ph].
%%CITATION = doi:10.1016/j.physletb.2012.02.013;%%
%409 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Degrassi:2012ry}
\bibitem{Degrassi:2012ry}
G.~Degrassi, S.~Di Vita, J.~Elias-Miro, J.~R.~Espinosa, G.~F.~Giudice, G.~Isidori and A.~Strumia,
%``Higgs mass and vacuum stability in the Standard Model at NNLO,''
JHEP {\bf 1208} (2012) 098
%doi:10.1007/JHEP08(2012)098
arXiv:1205.6497 [hep-ph].
%%CITATION = doi:10.1007/JHEP08(2012)098;%%
%1096 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Buttazzo:2013uya}
\bibitem{Buttazzo:2013uya}
D.~Buttazzo, G.~Degrassi, P.~P.~Giardino, G.~F.~Giudice, F.~Sala, A.~Salvio and A.~Strumia,
%``Investigating the near-criticality of the Higgs boson,''
JHEP {\bf 1312} (2013) 089
%doi:10.1007/JHEP12(2013)089
arXiv:1307.3536 [hep-ph].
%%CITATION = doi:10.1007/JHEP12(2013)089;%%
%882 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Espinosa:2007qp}
\bibitem{Espinosa:2007qp}
J.~R.~Espinosa, G.~F.~Giudice and A.~Riotto,
%``Cosmological implications of the Higgs mass measurement,''
JCAP {\bf 0805} (2008) 002
%doi:10.1088/1475-7516/2008/05/002
arXiv:0710.2484 [hep-ph].
%%CITATION = doi:10.1088/1475-7516/2008/05/002;%%
%274 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Enqvist:2014bua}
\bibitem{Enqvist:2014bua}
K.~Enqvist, T.~Meriniemi and S.~Nurmi,
%``Higgs Dynamics during Inflation,''
JCAP {\bf 1407} (2014) 025
%doi:10.1088/1475-7516/2014/07/025
arXiv:1404.3699 [hep-ph].
%%CITATION = doi:10.1088/1475-7516/2014/07/025;%%
%78 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Shkerin:2015exa}
\bibitem{Shkerin:2015exa}
A.~Shkerin and S.~Sibiryakov,
%``On stability of electroweak vacuum during inflation,''
Phys.\ Lett.\ B {\bf 746} (2015) 257
%doi:10.1016/j.physletb.2015.05.012
arXiv:1503.02586 [hep-ph].
%%CITATION = doi:10.1016/j.physletb.2015.05.012;%%
%45 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Lebedev:2012zw}
\bibitem{Lebedev:2012zw} 
O.~Lebedev,
%``On Stability of the Electroweak Vacuum and the Higgs Portal,''
Eur.\ Phys.\ J.\ C {\bf 72}, 2058 (2012)
% doi:10.1140/epjc/s10052-012-2058-2
[arXiv:1203.0156 [hep-ph]].
%%CITATION = doi:10.1140/epjc/s10052-012-2058-2;%%
%155 citations counted in INSPIRE as of 25 Aug 2018


%\cite{Kearney:2015vba}
\bibitem{Kearney:2015vba}
J.~Kearney, H.~Yoo and K.~M.~Zurek,
%``Is a Higgs Vacuum Instability Fatal for High-Scale Inflation?,''
Phys.\ Rev.\ D {\bf 91} (2015) no.12,  123537
%doi:10.1103/PhysRevD.91.123537
arXiv:1503.05193 [hep-th].
%%CITATION = doi:10.1103/PhysRevD.91.123537;%%
%63 citations counted in INSPIRE as of 24 Jan 2019

%\cite{Espinosa:2015qea}
\bibitem{Espinosa:2015qea}
J.~R.~Espinosa, G.~F.~Giudice, E.~Morgante, A.~Riotto, L.~Senatore, A.~Strumia and N.~Tetradis,
%``The cosmological Higgstory of the vacuum instability,''
JHEP {\bf 1509} (2015) 174
%doi:10.1007/JHEP09(2015)174
arXiv:1505.04825 [hep-ph].
%%CITATION = doi:10.1007/JHEP09(2015)174;%%
%150 citations counted in INSPIRE as of 24 Jan 2019

%\cite{EliasMiro:2012ay}
\bibitem{EliasMiro:2012ay}
J.~Elias-Miro, J.~R.~Espinosa, G.~F.~Giudice, H.~M.~Lee and A.~Strumia,
%``Stabilization of the Electroweak Vacuum by a Scalar Threshold Effect,''
JHEP {\bf 1206} (2012) 031
%doi:10.1007/JHEP06(2012)031
[arXiv:1203.0237 [hep-ph]].
%%CITATION = doi:10.1007/JHEP06(2012)031;%%
%236 citations counted in INSPIRE as of 28 Aug 2018

%\cite{Felder:2000hr}
\bibitem{Felder:2000hr}
G.~N.~Felder and L.~Kofman,
%``The Development of equilibrium after preheating,''
Phys.\ Rev.\ D {\bf 63} (2001) 103503
%doi:10.1103/PhysRevD.63.103503
[hep-ph/0011160].
%%CITATION = doi:10.1103/PhysRevD.63.103503;%%
%104 citations counted in INSPIRE as of 20 May 2018


\bibitem{Dodel}
``Modern Cosmology'' text by Scott Dodelson \
Academic Press Publication




  
  

  
  %\cite{McKellar:1992ja}
\bibitem{McKellar:1992ja} 
  B.~H.~J.~McKellar and M.~J.~Thomson,
  %``Oscillating doublet neutrinos in the early universe,''
  Phys.\ Rev.\ D {\bf 49}, 2710 (1994).
  %doi:10.1103/PhysRevD.49.2710
  %%CITATION = doi:10.1103/PhysRevD.49.2710;%%
  %176 citations counted in INSPIRE as of 25 Aug 2018
  
  %\cite{Sigl:1992fn}
\bibitem{Sigl:1992fn} 
  G.~Sigl and G.~Raffelt,
  %``General kinetic description of relativistic mixed neutrinos,''
  Nucl.\ Phys.\ B {\bf 406}, 423 (1993).
 % doi:10.1016/0550-3213(93)90175-O
  %%CITATION = doi:10.1016/0550-3213(93)90175-O;%%
  %397 citations counted in INSPIRE as of 25 Aug 2018
  
  %\cite{Jacques:2013xr}
\bibitem{Jacques:2013xr}
T.~D.~Jacques, L.~M.~Krauss and C.~Lunardini,
%``Additional Light Sterile Neutrinos and Cosmology,''
Phys.\ Rev.\ D {\bf 87} (2013) no.8,  083515
Erratum: [Phys.\ Rev.\ D {\bf 88} (2013) no.10,  109901]
%doi:10.1103/PhysRevD.87.083515, 10.1103/PhysRevD.88.109901
[arXiv:1301.3119 [astro-ph.CO]].
%%CITATION = doi:10.1103/PhysRevD.87.083515, 10.1103/PhysRevD.88.109901;%%
%43 citations counted in INSPIRE as of 26 Jun 2018

%\cite{Chu:2015ipa}
 \bibitem{Chu:2015ipa}
 X.~Chu, B.~Dasgupta and J.~Kopp,
 %``Sterile neutrinos with secret interactions—lasting friendship with cosmology,''
 JCAP {\bf 1510} (2015) no.10,  011
 %doi:10.1088/1475-7516/2015/10/011
 [arXiv:1505.02795 [hep-ph]].
 %%CITATION = doi:10.1088/1475-7516/2015/10/011;%%
 %38 citations counted in INSPIRE as of 03 Jul 2018
 
 %\cite{Chu:2018gxk}
 \bibitem{Chu:2018gxk}
 X.~Chu, B.~Dasgupta, M.~Dentler, J.~Kopp and N.~Saviano,
 %``Sterile Neutrinos with Secret Interactions -- Cosmological Discord?,''
 arXiv:1806.10629 [hep-ph].
 %%CITATION = ARXIV:1806.10629;%%
 
 %\cite{Farzan:2002wx}
 \bibitem{Farzan:2002wx}
 Y.~Farzan,
 %``Bounds on the coupling of the Majoron to light neutrinos from supernova cooling,''
 Phys.\ Rev.\ D {\bf 67} (2003) 073015
% doi:10.1103/PhysRevD.67.073015
 [hep-ph/0211375].
 %%CITATION = doi:10.1103/PhysRevD.67.073015;%%
 %72 citations counted in INSPIRE as of 29 Aug 2018

%\cite{Heurtier:2016otg}
\bibitem{Heurtier:2016otg}
L.~Heurtier and Y.~Zhang,
%``Supernova Constraints on Massive (Pseudo)Scalar Coupling to Neutrinos,''
JCAP {\bf 1702} (2017) no.02,  042
%doi:10.1088/1475-7516/2017/02/042
[arXiv:1609.05882 [hep-ph]].
%%CITATION = doi:10.1088/1475-7516/2017/02/042;%%
%8 citations counted in INSPIRE as of 03 Jul 2018



 
 %\cite{Felder:2000hq}
\bibitem{Felder:2000hq} 
  G.~N.~Felder and I.~Tkachev,
  %``LATTICEEASY: A Program for lattice simulations of scalar fields in an expanding universe,''
  Comput.\ Phys.\ Commun.\  {\bf 178}, 929 (2008)
  %doi:10.1016/j.cpc.2008.02.009
  [hep-ph/0011159].
  %%CITATION = doi:10.1016/j.cpc.2008.02.009;%%
  %130 citations counted in INSPIRE as of 19 Mar 2018



%\cite{Hardy:2017wkr}
\bibitem{Hardy:2017wkr}
E.~Hardy and J.~Unwin,
%``Symmetric and Asymmetric Reheating,''
JHEP {\bf 1709} (2017) 113
%doi:10.1007/JHEP09(2017)113
[arXiv:1703.07642 [hep-ph]].
%%CITATION = doi:10.1007/JHEP09(2017)113;%%
%9 citations counted in INSPIRE as of 29 Jun 2018

%\cite{Hyde:2015gwa}
\bibitem{Hyde:2015gwa}
J.~M.~Hyde,
%``Sensitivity of gravitational waves from preheating to a scalar field’s interactions,''
Phys.\ Rev.\ D {\bf 92} (2015) no.4,  044026
%doi:10.1103/PhysRevD.92.044026
[arXiv:1502.07660 [hep-ph]].
%%CITATION = doi:10.1103/PhysRevD.92.044026;%%
%2 citations counted in INSPIRE as of 29 Jun 2018

%\cite{Dolgov:1996fp}
\bibitem{Dolgov:1996fp} 
  A.~D.~Dolgov, S.~Pastor, J.~C.~Romao and J.~W.~F.~Valle,
  %``Primordial nucleosynthesis, Majorons and heavy tau neutrinos,''
  Nucl.\ Phys.\ B {\bf 496}, 24 (1997)
  %doi:10.1016/S0550-3213(97)00213-7
  [hep-ph/9610507].
  %%CITATION = doi:10.1016/S0550-3213(97)00213-7;%%
  %30 citations counted in INSPIRE as of 25 Aug 2018

%--------------------------------------------------------
%\cite{lite}
\bibitem{lite}
A.~Suzuki {\it et al.} [LiteBIRD Collaboration],
arXiv:1801.06987 [astro-ph.IM]

%A.~Suzuki

%\cite{DiValentino:2016foa}
\bibitem{DiValentino:2016foa}
E.~Di Valentino {\it et al.} [CORE Collaboration],
%``Exploring cosmic origins with CORE: Cosmological parameters,''
JCAP {\bf 1804} (2018) 017
%doi:10.1088/1475-7516/2018/04/017
[arXiv:1612.00021 [astro-ph.CO]].
%%CITATION = doi:10.1088/1475-7516/2018/04/017;%%
%52 citations counted in INSPIRE as of 20 Aug 2018

%\cite{pixie}
\bibitem{pixie}
A.~Kogut {\it et al.} [PIXIE Collaboration],
arXiv:1105.2044  [astro-ph.CO].

%\cite{Abazajian:2016yjj}
\bibitem{Abazajian:2016yjj}
K.~N.~Abazajian {\it et al.} [CMB-S4 Collaboration],
%``CMB-S4 Science Book, First Edition,''
arXiv:1610.02743 [astro-ph.CO].
%%CITATION = ARXIV:1610.02743;%%
%316 citations counted in INSPIRE as of 20 Aug 2018

%\cite{cmbbharat}
\bibitem{cmbbharat}
\textit{http://cmb-bharat.in/wp-content/uploads/2018/06/cmb-bharat-rao-tp-es.pdf}

%\cite{Acciarri:2016smi}
\bibitem{Acciarri:2016smi}
R.~Acciarri {\it et al.} [MicroBooNE Collaboration],
%``Design and Construction of the MicroBooNE Detector,''
JINST {\bf 12} (2017) no.02,  P02017
%doi:10.1088/1748-0221/12/02/P02017
[arXiv:1612.05824 [physics.ins-det]].
%%CITATION = doi:10.1088/1748-0221/12/02/P02017;%%
%53 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Chauhan:2018dkd}
\bibitem{Chauhan:2018dkd} 
  B.~Chauhan and S.~Mohanty,
  %``Signature of Light Sterile Neutrinos at IceCube,''
  arXiv:1808.04774 [hep-ph].
  %%CITATION = ARXIV:1808.04774;%%
  
  %\cite{Choudhury:2018sbz}
\bibitem{Choudhury:2018sbz} 
  S.~Roy Choudhury and S.~Choubey,
  %``Constraining light sterile neutrino mass with the BICEP2/Keck Array 2014 B-mode polarization data,''
  arXiv:1807.10294 [astro-ph.CO].
  %%CITATION = ARXIV:1807.10294;%%
  
  
  %\cite{Guzzetti:2016mkm}
\bibitem{Guzzetti:2016mkm} 
  M.~C.~Guzzetti, N.~Bartolo, M.~Liguori and S.~Matarrese,
  %``Gravitational waves from inflation,''
  Riv.\ Nuovo Cim.\  {\bf 39}, no. 9, 399 (2016)
 % doi:10.1393/ncr/i2016-10127-1
  [arXiv:1605.01615 [astro-ph.CO]].
  %%CITATION = doi:10.1393/ncr/i2016-10127-1;%%
  %47 citations counted in INSPIRE as of 29 Aug 2018


%\cite{Boyarsky:2018tvu}
 \bibitem{Boyarsky:2018tvu} A.~Boyarsky, M.~Drewes, T.~Lasserre, S.~Mertens and O.~Ruchayskiy, %``Sterile Neutrino Dark Matter,''
arXiv:1807.07938 [hep-ph].
%%CITATION = ARXIV:1807.07938;%%
%1 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Herms:2018ajr}
 \bibitem{Herms:2018ajr} J.~Herms, A.~Ibarra and T.~Toma, %``A new mechanism of sterile neutrino dark matter production,''
JCAP {\bf 1806}, no. 06, 036 (2018)
%doi:10.1088/1475-7516/2018/06/036
[arXiv:1802.02973 [hep-ph]].
%%CITATION = doi:10.1088/1475-7516/2018/06/036;%%
%4 citations counted in INSPIRE as of 20 Aug 2018

%\cite{Hochberg:2014kqa}
\bibitem{Hochberg:2014kqa} 
  Y.~Hochberg, E.~Kuflik, H.~Murayama, T.~Volansky and J.~G.~Wacker,
  %``Model for Thermal Relic Dark Matter of Strongly Interacting Massive Particles,''
  Phys.\ Rev.\ Lett.\  {\bf 115}, no. 2, 021301 (2015)
  %doi:10.1103/PhysRevLett.115.021301
  [arXiv:1411.3727 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.115.021301;%%
  %109 citations counted in INSPIRE as of 21 Aug 2018

%\cite{Hochberg:2014dra}
\bibitem{Hochberg:2014dra} 
  Y.~Hochberg, E.~Kuflik, T.~Volansky and J.~G.~Wacker,
  %``Mechanism for Thermal Relic Dark Matter of Strongly Interacting Massive Particles,''
  Phys.\ Rev.\ Lett.\  {\bf 113}, 171301 (2014)
  %doi:10.1103/PhysRevLett.113.171301
  [arXiv:1402.5143 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.113.171301;%%
  %193 citations counted in INSPIRE as of 21 Aug 2018
 
  
%\cite{Cline:1991zb}
\bibitem{Cline:1991zb} 
  J.~M.~Cline,
  %``Constraints on almost Dirac neutrinos from neutrino - anti-neutrino oscillations,''
  Phys.\ Rev.\ Lett.\  {\bf 68}, 3137 (1992).
  %doi:10.1103/PhysRevLett.68.3137
  %%CITATION = doi:10.1103/PhysRevLett.68.3137;%%
  %86 citations counted in INSPIRE as of 26 Apr 2018
  
  
  %\cite{Notzold:1987ik}
\bibitem{Notzold:1987ik} 
  D.~Notzold and G.~Raffelt,
  %``Neutrino Dispersion at Finite Temperature and Density,''
  Nucl.\ Phys.\ B {\bf 307}, 924 (1988).
 % doi:10.1016/0550-3213(88)90113-7
  %%CITATION = doi:10.1016/0550-3213(88)90113-7;%%
  %408 citations counted in INSPIRE as of 26 Apr 2018
  
  %\cite{Nieves:2018vxl}
\bibitem{Nieves:2018vxl} 
  J.~F.~Nieves and S.~Sahu,
  %``Neutrino effective potential in a fermion and scalar background,''
  arXiv:1808.01629 [hep-ph].
  %%CITATION = ARXIV:1808.01629;%%
  
  %\cite{Quimbay:1995jn}
\bibitem{Quimbay:1995jn} 
  C.~Quimbay and S.~Vargas-Castrillon,
  %``Fermionic dispersion relations in the standard model at finite temperature,''
  Nucl.\ Phys.\ B {\bf 451}, 265 (1995)
  %doi:10.1016/0550-3213(95)00298-7
  [hep-ph/9504410].
  %%CITATION = doi:10.1016/0550-3213(95)00298-7;%%
  %32 citations counted in INSPIRE as of 26 Apr 2018
  
  %\cite{Weldon:1982bn}
\bibitem{Weldon:1982bn} 
  H.~A.~Weldon,
  %``Effective Fermion Masses of Order gT in High Temperature Gauge Theories with Exact Chiral Invariance,''
  Phys.\ Rev.\ D {\bf 26}, 2789 (1982).
  %doi:10.1103/PhysRevD.26.2789
  %%CITATION = doi:10.1103/PhysRevD.26.2789;%%
  %490 citations counted in INSPIRE as of 09 Jun 2018






\end{thebibliography}  
